A Precision Drone Landing System using Visual and IR Fiducial Markers and a Multi-Payload Camera

We propose a method for autonomous precision drone landing with fiducial markers and a gimbal-mounted, multi-payload camera with wide-angle, zoom, and IR sensors. The method has minimal data requirements; it depends primarily on the direction from the drone to the landing pad, enabling it to switch dynamically between the camera's different sensors and zoom factors, and minimizing auxiliary sensor requirements. It eliminates the need for data such as altitude above ground level, straight-line distance to the landing pad, fiducial marker size, and 6 DoF marker pose (of which the orientation is problematic). We leverage the zoom and wide-angle cameras, as well as visual April Tag fiducial markers to conduct successful precision landings from much longer distances than in previous work (168m horizontal distance, 102m altitude). We use two types of April Tags in the IR spectrum - active and passive - for precision landing both at daytime and nighttime, instead of simple IR beacons used in most previous work. The active IR landing pad is heated; the novel, passive one is unpowered, at ambient temperature, and depends on its high reflectivity and an IR differential between the ground and the sky. Finally, we propose a high-level control policy to manage initial search for the landing pad and subsequent searches if it is lost - not addressed in previous work. The method demonstrates successful landings with the landing skids at least touching the landing pad, achieving an average error of 0.19m. It also demonstrates successful recovery and landing when the landing pad is temporarily obscured.

==> sections/discussion.tex <==
The system accomplishes successful landings with an average error of 0.19m.
With the zoom camera, the system can recognize the visual landing pad and carry out successful
autonomous landings from long distances,
but since the \gls{IR} camera does not have an optical zoom, its range is more limited.
The active \gls{IR} landing pad
provides consistent performance and is clearly recognizable.
The passive \gls{IR} landing pad reflects the drone's IR radiation, % back to the camera,
causing occlusion when the drone is horizontally aligned and at low altitudes,
which necessitates the \emph{commit} state (limiting the landing accuracy),
but it requires no power source.
The performance of the passive \gls{IR} landing pad may be weather-dependent
and requires further testing.
The system is able to recover from detection losses by zooming out, ascending,
or restarting the search process.
Since the system follows the same control policy for all landing pads, the only major difference in
performance is the maximum detection distance.

